In-Network Processing Acoustic Data for Anomaly Detection in Smart Factory

Modern manufacturing is now deeply integrating new technologies such as 5G, Internet-of-things (IoT), and cloud/edge computing to shape manufacturing to a new level -- Smart Factory. Autonomic anomaly detection (e.g., malfunctioning machines and hazard situations) in a factory hall is on the list and expects to be realized with massive IoT sensor deployments. In this paper, we consider acoustic data-based anomaly detection, which is widely used in factories because sound information reflects richer internal states while videos cannot; besides, the capital investment of an audio system is more economically friendly. However, a unique challenge of using audio data is that sounds are mixed when collecting thus source data separation is inevitable. A traditional way transfers audio data all to a centralized point for separation. Nevertheless, such a centralized manner (i.e., data transferring and then analyzing) may delay prompt reactions to critical anomalies. We demonstrate that this job can be transformed into an in-network processing scheme and thus further accelerated. Specifically, we propose a progressive processing scheme where data separation jobs are distributed as microservices on intermediate nodes in parallel with data forwarding. Therefore, collected audio data can be separated 43.75% faster with even less total computing resources. This solution is comprehensively evaluated with numerical simulations, compared with benchmark solutions, and results justify its advantages.

==> backup/background.tex <==
\section{Background}\label{sec:background}
\comment{ATTENTION: to be re-written to fit to the story line.}

\subsection{Blind Source Separation}
\acrfull{bss}~\cite{comon2010handbook} is the process of recovering source signals from the mixture of observed ones.
Assume that $n$ acoustic sensors record acoustic signals from $n$ sources $\mathbf{S}$. The observed mixture of signals at each sensor, throughout $m$ time slots, is the addition of $n$ acoustic components from sources over that period.
The observed mixtures, denoted as $\mathbf{X}$, at each time instant is generated as a linear combination of the sources, the mixing process is presented as a mixing matrix $\mathbf{A}$.
% The size of $\mathbf{X}$ usually is enormous since acoustic signals are often sampled with tens of thousands of samples per second.
% Furthermore, typical \ac{iot} setup consists of a large number of $k$ of sensors, which exacerbates the length of observed data and the mixing matrix's size.
% Even though the number of observers $k$ can be more significant than the number of sources $n$ to perform \ac{bss}, $k$ should equal to $n$, for two reasons.
% First, a minimum number of observers is resource-efficient for both transmission and computation.
% Second and more importantly, the $n \times n$ square matrix is the smallest possible $n$-rank matrix, which is required for $\mathbf{A}$ to be invertible~\cite{hyvarinen1999fast}.
The mixing model can be understood as a function $\mathcal{M}$:
\begin{equation}\label{eq:bss}
    \textbf{X} = \mathcal{M}(\textbf{A}, \textbf{S}) = \textbf{A} \times \textbf{S},
\end{equation}
where $\textbf{A}$ is the mixing matrix.

\begin{figure}[t!]
\centerline{\includegraphics[width=\columnwidth]{figures/BSS_Model.pdf}}
\caption{Blind Source Separation.\comment{place holder}}
\label{fig:modelBSS}
\end{figure}
The task of the given \ac{bss} in~\cref{fig:modelBSS} is to estimate the source signals $\hat{\textbf{S}}$ by multiplying the observed mixtures with a separation matrix $\mathbf{W}$, which is an inverse of the mixing matrix, as follows:
\begin{equation}\label{eq:ica}
    \hat{\textbf{S}} = \mathcal{S}(\textbf{W}, \textbf{X}) = \textbf{A}^{-1} \textbf{X} = \textbf{W} \times \textbf{X}.
\end{equation}

\subsection{Processing Latency and Accuracy of Independent Component Analysis}
One of the well-known methods to estimate the separation matrix $\mathbf{W}$ is called \ac{ica}. 
Conventional ICA-based algorithms, such as FastICA~\cite{hyvarinen1999fast}, maximizes the non-gaussianity of observed data to separate the mixtures.
% Newton's Iteration can approximate the process of solving the non-gaussianity maximization.
The optimization of maximizing the non-gaussianity can be solved as an approximation of Newton's Iteration $\mathcal{N}$:
\begin{equation}\label{eq:newton_def}
    (\textbf{W}_{i}, \Delta_i) = \mathcal{N}(\textbf{X}, \textbf{W}_{i-1}), i \in \mathbb{N},
\end{equation}
where $\textbf{X}$ is the given mixture data, $\textbf{W}_{i}$ is the estimation of separation matrix in the $i$-th iteration.
$\Delta_i$ is the difference of $i$-th guessed $\textbf{W}_{i}$ to the previous $\textbf{W}_{i-1}$:
\begin{equation}\label{eq:diff_def}
    \Delta_i = \mathcal{D}(\textbf{W}_{i}, \textbf{W}_{i-1}) = \textbf{W}_{i} \times \textbf{W}_{i-1}^T - \textbf{I}, i \in \mathbb{N}.
\end{equation}
Newton's Iteration updates the separation matrix in every iteration towards a convergence point resulting in a correct separation of source signals.
In a robust implementation of Newton's Iteration, it is common to set a desired tolerance $Tol$.
Therefore, convergence $\mathcal{C}$ in the context of FastICA means that the difference $\Delta_i$ in the current iteration is within the desired tolerance $Tol$:
\begin{equation}\label{eq:convergence}
    \mathcal{C}(\Delta_i, Tol) = 
    \begin{cases}
        False,  & \Delta_i \geqslant Tol, i \in \mathbb{N},\\
        True, & \Delta_i < Tol, i \in \mathbb{N}.
    \end{cases}
\end{equation}

Under ideal cases, it is recommended to use all available data to obtain the most accurate separated sources, however the computation demanding can be challenging. 
Although the processing can be speeded up by using a small subset of the available data, it can affect the accuracy of the separation significantly.
This tricky trade-off has led to the development of Adaptive extraction-based Independent Component Analysis (AeICA)~\cite{Wu2012Adaptive} based on optimizing data extraction, to reduce traditional ICA algorithms' computation demand.
One step of Newton's Iteration only needs a subset of the original data, hence a partial Newton's Iteration reduces the need for computing demanding.
Therefore, AeICA accelerates the separation with high accuracy by two main improvements.
First, it extracts subset data for each iteration and exploits an adjusted convergence tolerance, reducing the processing latency. 
Second, AeICA uses an adaptive extraction distance to increase the amount of extracted data after each iteration, guaranteeing a reliable separation quality.

\comment{However, the adaptive extraction distance and convergence tolerance are based on the initial determined convergence tolerance and sometimes could be unstable from time to time, while in practice the signal is not homogeneous, resulting in deviations between the optimal value and the theoretical calculation.}

==> backup/experimental_design.tex <==
\section{Experiment Setup and Metrics}\label{sec:experimental_design}
In this section, we describe our experimental setup.
First, we picked a data set consisting of machine sounds and set up three network scenarios with different computational capabilities, which will be elaborated in\cref{subsec:evaluation_setup}.
In addition, we chose the most relevant current technologies as baseline and will compare them with the support of two metrics introduced in~\cref{subsec:evaluation_metrics}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% date set %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Setup}\label{subsec:evaluation_setup}
In our evaluation, we used the realistic dataset MIMII~\cite{Purohit_DCASE2019_01}.
It is a widely used acoustic data set for malfunctioning industrial machine inspection, containing 26092 normal and anomalous operating acoustic segments from four types of real machines: valves (V), pumps (P), fans (F), and slide rails (S).
Each acoustic segment is a single-channel 10-second acoustic data with a sampling rate of $16k~Hz$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% setup %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Experimental Setup}\label{subsec:evaluation_setup}
Based on this dataset, we set these four types of machines as the monitored objects.
In each round of experiments, a $4 \times 4$ mixing matrix $\mathbf{A}$ is generated following normal distribution $\mathcal{N}(0,1)$ to simulate the diverse interference among the monitored objects.
Meanwhile, four acoustic IoT devices were used to sense the mixed data, each collect $m = 16k~Hz \times 10s = 160k$ length data.
As shown in Fig. \comment{with computing as network function deployment figure in the future SOLUTION section}, these sensed data are transmitted by the client into the network and processed on the network nodes.
Each network node performed an extraction-based separation process. \comment{A proper noun is needed to refer to the partial separation operation based on extracted data, which will be defined in the SOLUTION section.}
After all network nodes are used to perform the separation task, the remaining separation tasks are processed by the server.
% At last, the server obtains the original acoustic signal of each machine.

We set up three different network scenarios: network with zero computational capability (node = 0), network with moderate computational capability (node = 7), and network with high computational capability (node = 15).
For the baseline systems, we choose the most relevant methods: AeICA and FastICA
It is important to note that FastICA can only be deployed on a single device due to its non-distributable nature.
Therefore, PICA, AeICA, and FastICA are equivalent in the scenario where the network has zero computational capability, but only server performs the separation task.

We implemented the separation functions in Python.
All sources used in our experiments are publicly available~\cite{innetworkbss}, and the experiments are reproducible on a single \ac{cots} server.
For each configuration of a network setup, we performed 50 measurements in which the client sends the mixture matrix to the server.
We calculated the mean results together with their 95\% confidence intervals. 
For the overall experiment, we employ a \ac{cots} server with an i7-6700T CPU with 16GB RAM using Ubuntu 18.04 LTS.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% metrics %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Metrics}\label{subsec:evaluation_metrics}
\subsubsection{Processing Time}
The processing time $t_p$ was measured by using the python module \texttt{time} with a precision of 1 microsecond ($\mu s$).
It covers the data processing time in the entire network, namely from the moment the data enters the network via the client until the moment the server obtains the separated source audio data.

\subsubsection{Processing Accuracy}
The \ac{sdr} metric is commonly used to evaluate source separation performance and is defined as:
\begin{equation}\label{eq:sdr}
    \ac{sdr} = 10\log_{10} \frac{\|s_{target}\|^2}{\|e_{interf} + e_{noise} + e_{artif}\|^2},
\end{equation}
where $s_{target}$ is the true source signals with an allowed distortion, and $e_{interf}$, $e_{noise}$ and $e_{artif}$ are the interference, noise and artifacts errors respectively~\cite{vincent2006performance}.
We use the open-source application BSS Eval Toolbox~\cite{stoter20182018} to calculate the \ac{sdr}.

\subsubsection{Distance to Final Separation}
Cosine distance $D_i$ in the~\cref{eq:define_cosin_distance} was used to indicate the distance of the separation matrix $\mathbf{W}_i$ computed by the $i$-th network node from the final separation matrix $\textbf{W} = \textbf{A}^{-1}$:
\begin{equation}\label{eq:define_cosin_distance}
    D_i = \frac{\textbf{W}_{i} \cdot \textbf{W}}{\|\textbf{W}_{i}\|_2 \|\textbf{W}\|_2 }.
\end{equation}
The larger the distance $D_i$, the more inaccurate the separation matrix calculated by the $i$-th network node.




==> backup/introduction.tex <==
\section{Introduction}\label{sec:introduction}
%\xxcmt{PREVIEW VERSION ONLY! (Storyline and its presentation will change.)}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% motivation %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Contemporary industry is in the dawn of a fourth revolution towards full digitization and intelligence. This means a deep integration of emerging technologies such as 5G network, Internet-of-things, artificial intelligence (AI) and cloud computing. Among these, industry IoT devices will act as both a data collector and the ultimate actuators of a remote intelligent computing agent closing the full control loop to realize fully autonomic factory operations. With the increasingly scale and complexity of a factory, massive industry IoT devices will be deployed. Therefore, future smart factory heavily relies on efficient data analysis solutions consuming massive data gathered from the IoT devices for decision making processes~\xxcmt{add citations please}.

A critical operation task in manufacturing is so-called ``anomaly detection'', which aims to detect the machine malfunctioning on the production line as soon as possible, in order to prevent the machines and/or the products from any serious damage and economy lost. In the past, this detection was manually done by allocating on-site human inspectors. Slowly, on-site inspectors were replaced by remote inspectors monitoring on screens. In the future, such inspection will be done  by intelligent agents through analyzing gathered sensing data from IoT devices equipped on the machines monitored and necessary reaction will be taken autonomously without human intervention.

For anomaly detection, comparing with video data, acoustic data is sometime more informational effective. One reason is that video data simply lacks such a direct reflection of the internal of a machine. In fact, for a long, acoustic signals are long being used by experienced workers, who can directly judge whether or not a machine works properly from the sound of a running machine. Another reason is that an acoustic sensing device is much cheaper than a professional camera thus more friendly to capitial investments and easy maintenance. Therefore, in the future smart factory era, acoustic data processing for anomaly detection will also play an important role in smart factory. \xxcmt{add citations please}

%With the development of the Internet of Things (IoT), humans and objects are integrated into a unified cyber-physical system, which allows the utilization of sensory data to permeate smart manufacturing (Industry 4.0).
%These sensory data in IIoT are often characterized by high volume, diversity, and variety. Therefore, relevant data analysis services are arising in IIoT networks to enable intelligent synthesis and efficient utilization of the aggregated data.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% problem %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Considering the nature of the two types of data signals (video and audio), video data is naturally separated by individual cameras. Unfortunately, this is not the case for acoustic data because the audio sources interfere each other. This means that an autonomic anomaly detection system based on acoustic data usually requires to restore the original source data from interfered data quickly enough, then a judgment can be made. 

To process the data gathered from all IoT sensors, a popular/conventional way is to first one-time transfer all data back to a compute node at remote (e.g. in a local cloud); after all data is ready, classical \ac{bss} algorithm (e.g. ICA-based methods~\cite{hyvarinen2000independent}, neural network-based methods~\cite{luo2019conv, 9367428}) can be executed to restore the original data. However, the limitations of the typical processing scheme are as follows:
\xxcmt{Here you discuss why one-time processing will be bad 1) ... and 2) ...}
Clearly, this may not fulfill the requirement of modern smart factory because the processing time could be long therefore necessarily prompt reactions could be delayed.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% solution %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this paper, we tackle this problem from another dimension: instead of focusing on improving the efficiency of a particular BSS algorithm itself, we were thinking if an in-network data processing can speed up the entire job, meanwhile keep the total resource consumption equivalent at least. In short, we propose an in-network data processing scheme where gathered IoT sensing data will be progressively processed by intermediate nodes along the forwarding path towards the final agent. 

The key idea is as follows: on every intermediate node, lightweight processing logic is deployed and spare compute resource (if available) is utilized; a predecessor node provides a half-cooked processing result to the successor node; in this step, with our modifications, we use the exiting ICA algorithm as a building block so that every node not only contributes to process the sensing data, but also provides a better starting point for the iteration on following nodes, resulting in overall faster convergence; when the last node (i.e. the actual remote agent) receives the data, it in parallel receives almost-ready processing result (i.e. the separated original source). In summary, our contributions can be summarize as follows:
\begin{enumerate}
		\item We propose an in-network data processing scheme for anomaly detection. Depending on the availability of intermediate nodes, such an scheme can largely improve the total processing time while maintain equivalent total resource consumption;
		\item We modify an existing ICA algorithm and integrate as a building block in our proposed scheme, so that the computing tasks can be distributed to intermediate nodes along the forwarding path to the actual decision-making agent at remote;
		\item We conduct extensive numerical simulations and results validate our proposed scheme, which indeed gives an anomaly detection solution for future smart factory but from a new dimension.
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% structure %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The rest of the paper is structured as follows.\xxcmt{Please modify the follow texts. I guess we need a prior art section but for discussing in-network computing rather than the algorithm anymore, a section for introducing the network architecture, then merge the current background as a subsection to YOUR SOLUTION section (must be shortened of course), then evalauation and conclusion}
\emph{First, \cref{sec:background} introduces the detection system and provides a description of the problem, after which, the proposed method is described in~\cref{sec:method}.
In~\cref{sec:experimental_design} we introduce the experimental setup and its metrics.
\cref{sec:results_analysis} covers the numerical evaluation and a discussion about our measurement results.
Finally, \cref{sec:conclusion} concludes our contribution and points out future research aspects.}

%In this paper, we propose a novel \ac{bss} algorithm for low-latency acoustic processing services: Progressive ICA (PICA).
%PICA follows the idea of data extraction and "divide and conquer", however, the extent of each divide and conquer is determined by the changing rate of occupancy, rather than the result of each occupancy.
%In this way, it retains the advantages of AeICA: optimizing processing latency and allowing in-network computing, while eliminating the constraint of sensitive initial extraction intervals.
%Thus, the proposed PICA effectively meets the need for low-latency speech processing services in IoT networks.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% gap %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Acoustic processing scenarios often require automatic~\ac{bss}, in order to transform the raw sensory data into clean acoustic data for subsequent analysis.
%In recent years, researchers have been investigating robust \ac{bss} techniques, such as ICA-based methods~\cite{hyvarinen2000independent}, and neural network-based methods~\cite{luo2019conv, 9367428}.
%However, due to the low latency requirement of acoustic processing services for industrial IoT, the service latency of \ac{bss} becomes a pressing challenge.
%In IoT networks, the service latency of \ac{bss} generally consists of two parts: data transmission latency and data processing latency.
%Despite the great success of communication technologies in reducing data transmission latency, data processing latency has not received sufficient attention at present.



%\xxcmt{all these will go to the solution section or prior art section, not in the introduction because the whole motivation is not these anymore}
%Since 2019, we have been working on reducing the processing latency of \ac{bss}. Because of the widespread use of ICA algorithms, we first proposed the CdICA~\cite{Wu2020} based on the fast \ac{bss} algorithm FastICA~\cite{hyvarinen1999fast}. 
%Compared to the reference system FastICA, the processing latency of CdICA for \ac{bss} is reduced, however, this approach requires specific deployment for IoT sensors.
%Later, in 2020, we proposed the AeICA~\cite{Wu2012Adaptive}, which has no specific requirements for hardware deployment and optimizes the processing latency significantly. 
%More importantly, in AeICA, since we introduced the idea of data extraction and "divide and conquer", it is possible for AeICA to be deployed and performed cooperatively on edge/fog devices, instead of on a delegated server, by using network virtualization technologies such as SDN and NFV.
%
%However, during the subsequent use, we noticed that AeICA is sensitive to the initial interval of data extraction, which is highly dependent on the probability distribution of the aggregated data.
%This decreases the robust of processing latency improvement, which in turn makes the difficulty of its practical applications. 
%%\comment{change this sentence}


%\comment{more emotion in this paragraph}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% proof %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> backup/introduction_backup.tex <==
\section{Introduction}\label{sec:introduction}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% motivation %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
With the development of the Internet of Things (IoT), humans and objects are integrated into a unified cyber-physical system, which allows the utilization of sensory data to permeate smart manufacturing (Industry 4.0).
These sensory data in IIoT are often characterized by high volume, diversity, and variety.
Therefore, relevant data analysis services are arising in IIoT networks to enable intelligent synthesis and efficient utilization of the aggregated data.
Compared with image data and other conventional data, acoustic data is characterized as being unaffected by light and coverage as well containing rich information, hence the acoustic processing scenarios in the context of smart manufacturing are gradually increasing.
In these scenarios, the demand for low latency services is increasingly prominent to ensure reliable and resilient production and controlling, such as human-machine voice interaction and acoustic anomaly detection in predictive maintenance. \comment{need citation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% problem %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Acoustic processing scenarios often require automatic \ac{bss}, in order to transform the raw sensory data into clean acoustic data for subsequent analysis.
In recent years, researchers have been investigating robust \ac{bss} techniques, such as ICA-based methods~\cite{hyvarinen2000independent}, and neural network-based methods~\cite{luo2019conv, 9367428}.
However, due to the low latency requirement of acoustic processing services for industrial IoT, the service latency of \ac{bss} becomes a pressing challenge.
In IoT networks, the service latency of \ac{bss} generally consists of two parts: data transmission latency and data processing latency.
Despite the great success of communication technologies in reducing data transmission latency, data processing latency has not received sufficient attention at present.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% gap %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Since 2019, we have been working on reducing the processing latency of \ac{bss}.
Because of the widespread use of ICA algorithms, we first proposed the CdICA~\cite{Wu2020} based on the fast \ac{bss} algorithm FastICA~\cite{hyvarinen1999fast}. 
Compared to the reference system FastICA, the processing latency of CdICA for \ac{bss} is reduced, however, this approach requires specific deployment for IoT sensors.
Later, in 2020, we proposed the AeICA~\cite{Wu2012Adaptive}, which has no specific requirements for hardware deployment and optimizes the processing latency significantly. 
More importantly, in AeICA, since we introduced the idea of data extraction and "divide and conquer", it is possible for AeICA to be deployed and performed cooperatively on edge/fog devices, instead of on a delegated server, by using network virtualization technologies such as SDN and NFV.
However, during the subsequent use, we noticed that AeICA is sensitive to the initial interval of data extraction, which is highly dependent on the probability distribution of the aggregated data.
This decreases the robust of processing latency improvement, which in turn makes the difficulty of its practical applications.\comment{change this sentence}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% solution %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this paper, we propose a novel \ac{bss} algorithm for low-latency acoustic processing services: Progressive ICA (PICA).
PICA follows the idea of data extraction and "divide and conquer", however, the extent of each divide and conquer is determined by the changing rate of occupancy, rather than the result of each occupancy.
In this way, it retains the advantages of AeICA: optimizing processing latency and allowing in-network computing, while eliminating the constraint of sensitive initial extraction intervals.
Thus, the proposed PICA effectively meets the need for low-latency speech processing services in IoT networks.\comment{more emotion in this paragraph}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% proof %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% structure %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The rest of the paper is structured as follows.
First, \cref{sec:background} introduces the detection system and provides a description of the problem, after which, the proposed method is described in~\cref{sec:method}.
In~\cref{sec:experimental_design} we introduce the experimental setup and its metrics.
\cref{sec:results_analysis} covers the numerical evaluation and a discussion about our measurement results.
Finally, \cref{sec:conclusion} concludes our contribution and points out future research aspects.

==> backup/method_backup.tex <==
\section{Our Solution: Progressive ICA}\label{sec:method}
\comment{ATTENTION: to be re-written to fit to the story line.}

In this section, we propose Progressive Independent Component Analysis (PICA), aiming to speed up the speed up the separation and to avoid the instability encountered by AeICA. 
\comment{split the following content into two subsections: general architecture, key step and its proof}

% \begin{figure*}[t!]
% \centerline{\includegraphics[width=.9\textwidth]{figures/architecture.pdf}}
% \caption{Architecture of Progressive ICA.\comment{draft}}
% \label{fig:architecture}
% \end{figure*}
% \subsection{Architecture}
Even though the source separation in ICA is an iterative process, we apply the divide-and-conquer approach, PICA decouples it into three main functionalities, namely \acrfull{de}, \acrfull{sme}, and \acrfull{dr}.
Altogether, DE extracts a small fraction of the observed mixture and sends it to SME.
Then, SME uses the fraction to estimate the separation matrix.
If the estimation result approaches the desired tolerance, then \ac{dr} starts reconstructing separated sources.
Otherwise, \ac{sme} requests \ac{de} to extract more data for the estimation.
\cref{fig:architecture} depicts the three main functionalities and their dependency as a flowchart.

\subsubsection{\acrlong{de}}
\ac{de} receives the mixture $\mathbf{X} \in \mathbb{R}^{n \times m}$ observed from $n$ sources throughout $m$ time slots.
The goal of DE is to down sample $\mathbf{X}$ and extract a minimum subset of it that allows for estimating successfully the separation matrix.  
To quickly converge to an optimal set, DE needs to start with a substantially large subset and increase it at a reasonable speed.
We characterize this process by an extraction distance parameter $\mu_i$, where $i$ is the iteration number of the extraction operations.
\ac{de} extracts every $\mu_i$-th column from $\mathbf{X}$ to form a new matrix:
\comment{equation}

Initially, $\mu_i$ starts with $\frac{m}{n}$.\comment{Description is not accurate, need to be updated, it's more about preprocessing.}
As long as the extracted matrix does not meet the tolerance condition, \ac{de} performs a new extraction iteration in which $\mu_{i+1}$ is reduced by half.
\ac{de} terminates when the extracted matrix meets the desired tolerance, or the extraction distance reaches zero, meaning to take the whole mixture matrix $\mathbf{X}$.

\subsubsection{\acrlong{sme}}
The goal of \ac{sme} is to estimate the separation matrix $\mathbf{W}$.
\ac{sme} applies the Newton's Iteration on the extracted data from \ac{de}, denoted by ${}_{\mu_i}\mathbf{X}$.
\ac{sme} terminates when the outcome of Newton's Iteration approaches the desired tolerance.
Since the procedure to calculate the separation matrix $\mathbf{W}$ is computation-intensive and can take a long time, \ac{sme} adds an intermediate step to check the reduction rate of gradient after each iterative operation:
\comment{equation}

If gradient reduction of the estimated separation matrix is sufficiently large, then \ac{sme} continues with Newton's iteration.
Only when the matrix ${}_{\mu_i}\mathbf{W}$ has a sufficiently reduced gradient, then SME checks its tolerance. We illustrate the process as the decision of ``Slow Gradient Reduction'' in~\cref{fig:architecture}:
\comment{mathematically explanation and proof, or we need a separated subsection to talk about this.}
When the rate of descent of $\Delta_i$ decreases, the iteration process in current extraction distance will jump out. The  slow gradient reduction jump out condition is thus defined as \comment{update this equation}:
\begin{equation}\label{eq:descent_jump_out}
    sum(\textbf{Tols}) <
    P_{break}*0.5*(max(\textbf{Tols})+\textbf{Tols}[-1])*size(\textbf{Tols})
\end{equation}

The gradient sufficiently reduced matrix ${}_{\mu_i}\mathbf{W}$ is verified if it meets the desired tolerance:
\begin{itemize}
    \item If ${}_{\mu_i}\mathbf{W}$ does not meet the desired tolerance, SME continues using this ${}_{\mu_i}\mathbf{W}$ in the next iteration. At the same time, \ac{sme} requests a larger ${}_{\mu_i}\mathbf{X}$ from \ac{de}. i.e., with an updated $\mu_i$.
    \item If ${}_{\mu_i}\mathbf{W}$ meets the desired tolerance, meaning that the separation matrix $\mathbf{W}$ has been found and used for reconstructing separated sources $\hat{\mathbf{S}}$.
\end{itemize}
\comment{bring the factor of $\mu_0$ in.}

\subsubsection{\acrlong{dr}}
\ac{dr} is responsible for reconstructing the separated sources $\hat{\mathbf{S}}$, which is the final step of the ICA process and is executed only once.
\ac{dr} performs a matrix multiplication between the observed mixture $\mathbf{X}$ and the final separation matrix $\mathbf{W}$. \ac{dr} then outputs the separated source signals.
While \ac{dr} requires a relatively small computing demand, its output data volume is significantly larger than that of its input data.

% \subsection{Backup}
% Like AeICA, PICA use small subsets of the available data to improve the speed of convergence, and then increase the size of the subset to lead the separation to a better accuracy. The difference is, the tolerances are based on the previous convergence speed and user determined tolerance, and the extraction distance in iterations are based on the previous calculation.

% The whole process of the algorithm is to achieve a more accurate W through progressive calculation, and then substitute the W into FastICA calculation to achieve acceleration. So the question is how to calculate the W more efficient and accuracy.

% \subsection{Convergence speed and the size of subset}

% According to the formula of Newton's Iteration $\mathcal{N}$ for FastICA in~\cite{hyvarinen1999fast} is thus defined as:
% \begin{equation}\label{eq:newton_iteration}
%     \begin{cases} 
%     \textbf{W}_{i+1} = & \mathit{E}\{\textbf{X} g(\textbf{W}_i^T \textbf{X})\} - \mathit{E}\{g^{\prime}(\textbf{W}_i^T \textbf{X})\}\textbf{W}_i, \\
%     \textbf{W}_{i+1} = & \frac{\textbf{W}_{i+1}}{\| \textbf{W}_{i+1} \|}.
%     \end{cases}
% \end{equation}

% $\Delta_i$ is the difference of $i$-th guessed $\textbf{W}_{i}$ to the previous $\textbf{W}_{i-1}$:
% \begin{equation}\label{eq:diff_def}
%     \Delta_i = \mathcal{D}(\textbf{W}_{i}, \textbf{W}_{i-1}) = \textbf{W}_{i} \times \textbf{W}_{i-1}^T - \textbf{I}, i \in \mathbb{N}.
% \end{equation}

% The convergence speed $\mathcal{V}_{convergence}$ of each iteration is:
% \begin{equation}\label{eq:v_convergence_def}
%     \begin{cases} 
%     \mathcal{V}_{convergence} = & \frac{\Delta_i}{ \mathcal{T}_{iteration}}, \\
%     \mathcal{T}_{iteration}  = & \frac{\Delta_i}{ \mathcal{T}_{\mathit{E}\{\textbf{X} g(\textbf{W}_i^T \textbf{X})\} - \mathit{E}\{g^{\prime}(\textbf{W}_i^T \textbf{X})\}\textbf{W}_i} + \mathcal{T}_{ \frac{\textbf{W}_{i+1}}{\| \textbf{W}_{i+1} \|}}}
%     \end{cases}
% \end{equation}


% It can be seen from the equation that the size of X only affects the accuracy of $\Delta_i$, and does not affect its size. While the time of $\mathcal{T}_{\mathit{E}\{\textbf{X} g(\textbf{W}_i^T \textbf{X})\} - \mathit{E}\{g^{\prime}(\textbf{W}_i^T \textbf{X})\}\textbf{W}_i}$ is proportional to the size of X. Thus, when the $\Delta_i$ from the subset is accuracy enough. The convergence speed can be increased with a small subset.

% However, the deviation of $\Delta_i$ is not negligible. Therefore, We need to gradually increase the subset to reduce the $\Delta_i$ bias. 

% \subsection{Convergence speed and saddle point}

% From~\cref{eq:diff_def}, the convergence speed is proportional to $\Delta_i$. Meanwhile the value of $\Delta_i$ is not invariant. In general, there will be a saddle point at which the Newton iteration rate is greatly reduced near the saddle point. For a faster convergence rate, we need methods to avoid the iterative process wasting much time around the saddle point.

% our solution is an additional slow gradient reduction jump out for each iteration. When the rate of descent of $\Delta_i$ decreases, the iteration process in current extraction distance will jump out. The  slow gradient reduction jump out condition is thus defined as:
% \begin{equation}\label{eq:descent_jump_out}
%     sum(\textbf{Tols}) <
%     P_{break}*0.5*(max(\textbf{Tols})+\textbf{Tols}[-1])*size(\textbf{Tols})
% \end{equation}

% ~\cref{eq:descent_jump_out} is not optimal. When the  


% we introduced a gradient descent jump-out and a new adaptive adjustment of the extraction distance to reduce the impact of the $\Delta_i$ bias.







% \subsection{Iteration on Subset}

==> backup/results_analysis_backup.tex <==
\section{Results} \label{sec:results_analysis}
In this section, we present and discuss the performance of PICA, by comparing with the baseline methods.
\cref{sec:latency_accuracy} shows the processing time and processing accuracy of PICA in three network scenarios, and \cref{sec:pica_steps} details the advancement of progressive analysis.

\subsection{Processing Latency and Accuracy}\label{sec:latency_accuracy}
% \begin{figure}[t!]
% \centerline{\includegraphics[width=\columnwidth]{figures/time.pdf}}
% \caption{Processing Latency.\comment{draft}}
% \label{fig:time}
% \end{figure}
\begin{figure}[t!]
\centerline{\includegraphics[width=\columnwidth]{figures/time_on_nodes.pdf}}
\caption{Processing time with different network computational capacities.}
\label{fig:time_on_nodes}
\end{figure}
\cref{fig:time_on_nodes} shows the processing time of the separation methods in different network scenarios.
It can be observed that PICA is able to utilize the network computational capability to accelerate the processing with maximum efficiency.
Overall, the utilization of network computational capability can reduce the processing time from ca. $85ms$ to ca. $50ms$, which is a $41.18\%$ decrease in processing time.
Moreover, the network resources affect the acceleration.
When node = 0, the network has zero computational capability, naturally all computational tasks are pushed to the server, thus the processing time optimization is not obtained.
With seven nodes providing computational capability, these nodes might be insufficient to perform all processing tasks, making some of the tasks to be shifted to the server. 
For node = 15 the network computational capability is sufficient to complete all processing tasks, so the algorithm is most efficient.
% FastICA, on the other hand, does not react to the computing capability provided by the network, and the time consumption is always the largest.


Meanwhile, we noticed the influence of the parameter initial separation interval $\mu_0$ on the acceleration performance. 
For PICA, with $\mu_0=1$, there is almost no acceleration because PICA utilizes only one node regardless of the network's computational capability. 
A subsequent update of the extraction interval $\mu_1$ becomes zero, which is equivalent to no extraction, but rather using all data for centralized processing on the server.
However, picking other $\mu_0$s in PICA quickly improves the acceleration performance, for example, in Figure 4, with $\mu_0=3$ the processing time can already be reduced to about 60ms.
However, in our baseline system, because of the sensitivity of AeICA to the initial extraction interval, even if the network computational capability are sufficient with node = 15, AeICA may just do meaningless extraction and computation on these nodes, wasting network resources and finally pushing the remaining processing tasks to the server.
Thus, it could be impossible to use the network computational capability to optimize the processing time, for example, this happens when $\mu_0 > 300$.
In extreme cases, this can increase the processing time.


% In~\cref{fig:time}, the processing latency of separating four 10s-long mixed sources is shown to verify the influence of the initial extraction interval on the speedup performance of the algorithm.
% It can be seen that the speedup performance of the proposed PICA is stable for different initial extraction intervals.
% The processing latency of PICA is about 50-60ms, which is approx. $50\%$ less than that of FastICA.
% In the baseline method FastICA, progressive analysis is not introduced, so its initial extraction interval is always 0, and the processing delay of FastICA is stable.
% However, because of the lack of progressive analysis, FastICA has a high processing latency of about 110ms overall.
% AeICA can achieve similar speedup performance as PICA only when the initial extraction interval is between 3 and 40.
% When the initial extraction interval is set larger, the processing delay is even higher than that of FastICA. 
% This makes it much more difficult to configure the system parameters when using AeICA.
% To conclude, PICA not only maintains a good performance of accelerated processing latency, but also its stable characteristics make it much less difficult to set system parameters in practical applications.
% In turn, it can provide fast and reliable services and reduce system management costs.

\begin{figure}[t!]
\centerline{\includegraphics[width=\columnwidth]{figures/sdr.pdf}}
\caption{Processing Accuracy.\comment{draft}}
\label{fig:sdr}
\end{figure}
\cref{fig:sdr} shows the processing accuracy \ac{sdr} of PICA, AeICA, and FastICA.
It is worth noting that the three methods achieve essentially the same processing accuracy.
This is because in the progressive analysis, the extraction of data at large intervals occurs only at points that are far from the separation convergence point ($D_i$), with the aim of quickly approaching the convergence point.
As the convergence point remains original, the correctness of the separation matrix can be guaranteed.

Although the earlier network nodes use a subset of data to quickly construct an inaccurate separation matrix $\mathbf{W}_i$, the successor network nodes use the $\mathbf{W}_i$ as a starting point to obtain a more accurate separation matrix with more data.
through the collaborative computing of these network nodes, the whole separation task can reach the original convergence point and achieve the equally accurate separation matrix, which in turn guarantees the processing accuracy.
The process of progressive analysis is presented in~\cref{sec:pica_steps} in more detail.

\subsection{Progressive Analysis}\label{sec:pica_steps}
\begin{figure}[t!]
\centerline{\includegraphics[width=\columnwidth]{figures/iteration_step.pdf}}
\caption{Iteration Steps.}
\label{fig:iteration_step}
\end{figure}
\cref{fig:iteration_step} shows the data extraction $\mu_0$, the distance from the convergence point $D_i$, and the current accuracy \ac{sdr} of PICA, AeICA, and FastICA, respectively.\comment{more content!!!}
